Block-to-Block Distribution Matching

In this work, binary block-to-block distribution matching is considered. m independent and uniformly distributed bits are mapped to n output bits resembling a target product distribution. A rate R is called achieved by a sequence of encoder-decoder pairs, if for m,n to infinity, (1) m/n approaches R, (2) the informational divergence per bit of the output distribution and the target distribution goes to zero, and (3) the probability of erroneous decoding goes to zero. It is shown that the maximum achievable rate is equal to the entropy of the target distribution. A practical encoder-decoder pair is constructed that provably achieves the maximum rate in the limit. Numerical results illustrate that the suggested system operates close to the limits with reasonable complexity. The key idea is to internally use a fixed-to-variable length matcher and to compensate underflow by random mapping and to cast an error when overflow occurs.

==> Makefile <==
PROJECT=block
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps\
*.ind *.idx *.ilg *.gls *.glo *.glg *.acn *.acr *.alg *.ist *.out\
*.thm
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib .*.xml


default:
	pdflatex -shell-escape $(PROJECT).tex;

clean:
	rm -f $(TMPFILES);

clean_pdf:
	rm -f $(PROJECT).pdf;

literatur:
	cp ../references/Dnc.bib ./;
	cp ../references/confs-jrnls.bib ./;
	cp ../references/IEEEabrv.bib ./;
	cp ../references/IEEEtran.cls ./;
	cp ../references/IEEEtran.bst ./;

final: clean clean_pdf
	pdflatex -shell-escape $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	bibtex $(PROJECT);
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;


